Parametric machines: a fresh approach to architecture search

Using tools from topology and functional analysis, we provide a framework where artificial neural networks, and their architectures, can be formally described. We define the notion of machine in a general topological context and show how simple machines can be combined into more complex ones. We explore finite- and infinite-depth machines, which generalize neural networks and neural ordinary differential equations. Borrowing ideas from functional analysis and kernel methods, we build complete, normed, infinite-dimensional spaces of machines, and we discuss how to find optimal architectures and parameters -- within those spaces -- to solve a given computational problem. In our numerical experiments, these kernel-inspired networks can outperform classical neural networks when the training dataset is small.

==> Figures/architecture2D.tex <==
\begin{tikzpicture}
\begin{axis}[title={2D network architecture}]
    \addplot[quiver={u={\thisrow{u}}, v={\thisrow{v}}}, -stealth]
        table[row sep={\\}]
        {
            x  y  u  v  \\
            1  0  -1  1  \\
            2  0  -1  4  \\
            3  0  -1  9  \\
            4  0  -1  16  \\
            5  0  -1  25  \\
            0  1  0  -1  \\
            1  1  -1  0  \\
            2  1  -1  3  \\
            3  1  -1  8  \\
            4  1  -1  15  \\
            5  1  -1  24  \\
            0  2  1  -1  \\
            1  2  0  -1  \\
            2  2  -1  2  \\
            3  2  -1  7  \\
            4  2  -1  14  \\
            5  2  -1  23  \\
            0  3  1  -1  \\
            1  3  0  -1  \\
            2  3  -1  1  \\
            3  3  -1  6  \\
            4  3  -1  13  \\
            5  3  -1  22  \\
            0  4  1  -1  \\
            1  4  0  -1  \\
            2  4  -1  0  \\
            3  4  -1  5  \\
            4  4  -1  12  \\
            5  4  -1  21  \\
            0  5  2  -1  \\
            1  5  1  -1  \\
            2  5  0  -1  \\
            3  5  -1  4  \\
            4  5  -1  11  \\
            5  5  -1  20  \\
            0  6  2  -1  \\
            1  6  1  -1  \\
            2  6  0  -1  \\
            3  6  -1  3  \\
            4  6  -1  10  \\
            5  6  -1  19  \\
            0  7  2  -1  \\
            1  7  1  -1  \\
            2  7  0  -1  \\
            3  7  -1  2  \\
            4  7  -1  9  \\
            5  7  -1  18  \\
            0  8  2  -1  \\
            1  8  1  -1  \\
            2  8  0  -1  \\
            3  8  -1  1  \\
            4  8  -1  8  \\
            5  8  -1  17  \\
            0  9  2  -1  \\
            1  9  1  -1  \\
            2  9  0  -1  \\
            3  9  -1  0  \\
            4  9  -1  7  \\
            5  9  -1  16  \\
            0  10  3  -1  \\
            1  10  2  -1  \\
            2  10  1  -1  \\
            3  10  0  -1  \\
            4  10  -1  6  \\
            5  10  -1  15  \\
            0  11  3  -1  \\
            1  11  2  -1  \\
            2  11  1  -1  \\
            3  11  0  -1  \\
            4  11  -1  5  \\
            5  11  -1  14  \\
            0  12  3  -1  \\
            1  12  2  -1  \\
            2  12  1  -1  \\
            3  12  0  -1  \\
            4  12  -1  4  \\
            5  12  -1  13  \\
            0  13  3  -1  \\
            1  13  2  -1  \\
            2  13  1  -1  \\
            3  13  0  -1  \\
            4  13  -1  3  \\
            5  13  -1  12  \\
            0  14  3  -1  \\
            1  14  2  -1  \\
            2  14  1  -1  \\
            3  14  0  -1  \\
            4  14  -1  2  \\
            5  14  -1  11  \\
            0  15  3  -1  \\
            1  15  2  -1  \\
            2  15  1  -1  \\
            3  15  0  -1  \\
            4  15  -1  1  \\
            5  15  -1  10  \\
            0  16  3  -1  \\
            1  16  2  -1  \\
            2  16  1  -1  \\
            3  16  0  -1  \\
            4  16  -1  0  \\
            5  16  -1  9  \\
            0  17  4  -1  \\
            1  17  3  -1  \\
            2  17  2  -1  \\
            3  17  1  -1  \\
            4  17  0  -1  \\
            5  17  -1  8  \\
            0  18  4  -1  \\
            1  18  3  -1  \\
            2  18  2  -1  \\
            3  18  1  -1  \\
            4  18  0  -1  \\
            5  18  -1  7  \\
            0  19  4  -1  \\
            1  19  3  -1  \\
            2  19  2  -1  \\
            3  19  1  -1  \\
            4  19  0  -1  \\
            5  19  -1  6  \\
            0  20  4  -1  \\
            1  20  3  -1  \\
            2  20  2  -1  \\
            3  20  1  -1  \\
            4  20  0  -1  \\
            5  20  -1  5  \\
            0  21  4  -1  \\
            1  21  3  -1  \\
            2  21  2  -1  \\
            3  21  1  -1  \\
            4  21  0  -1  \\
            5  21  -1  4  \\
            0  22  4  -1  \\
            1  22  3  -1  \\
            2  22  2  -1  \\
            3  22  1  -1  \\
            4  22  0  -1  \\
            5  22  -1  3  \\
            0  23  4  -1  \\
            1  23  3  -1  \\
            2  23  2  -1  \\
            3  23  1  -1  \\
            4  23  0  -1  \\
            5  23  -1  2  \\
            0  24  4  -1  \\
            1  24  3  -1  \\
            2  24  2  -1  \\
            3  24  1  -1  \\
            4  24  0  -1  \\
            5  24  -1  1  \\
            0  25  4  -1  \\
            1  25  3  -1  \\
            2  25  2  -1  \\
            3  25  1  -1  \\
            4  25  0  -1  \\
            5  25  -1  0  \\
        }
        ;
\end{axis}
\end{tikzpicture}

